Near-infrared spectroscopy of 5 ultra-massive galaxies at 1.7 < z < 2.7

We present the results of a pilot near-infrared (NIR) spectroscopic campaign of five very massive galaxies ($\log(\text{M}_\star/\text{M}_\odot)>11.45$) in the range of $1.7<z<2.7$. We measure an absorption feature redshift for one galaxy at $z_\text{spec}=2.000\pm0.006$. For the remaining galaxies, we combine the photometry with the continuum from the spectra to estimate continuum redshifts and stellar population properties. We define a continuum redshift ($z_{\rm cont}$ ) as one in which the redshift is estimated probabilistically using EAZY from the combination of catalog photometry and the observed spectrum. We derive the uncertainties on the stellar population synthesis properties using a Monte Carlo simulation and examine the correlations between the parameters with and without the use of the spectrum in the modeling of the spectral energy distributions (SEDs). The spectroscopic constraints confirm the extreme stellar masses of the galaxies in our sample. We find that three out of five galaxies are quiescent (star formation rate of $\lesssim 1 M_\odot~yr^{-1}$) with low levels of dust obscuration ($A_{\rm V} < 1$) , that one galaxy displays both high levels of star formation and dust obscuration (${\rm SFR} \approx 300 M_\odot~{\rm yr}^{-1}$, $A_{\rm V} \approx 1.7$~mag), and that the remaining galaxy has properties that are intermediate between the quiescent and star-forming populations.

==> texme <==
#!/bin/bash

set -e

if [ ! -z $2 ]
then
    echo $2
    # eventually change this to clean
fi


function check_py {
    python - <<END
print("$input")
END
}

input=$1
function fix_that_break {
    python - <<EOF
import re
orig = open('$input.bbl','r').read()
new = re.sub('\\mnr%\nas', 'mnras', orig)
open('$input.bbl', 'w').write(new)
EOF
}


echo "Compiling $1 ..."
pdflatex $1
bibtex $1

if [ $USER == efong01 ]
then
    fix_that_break 
fi

pdflatex $1
pdflatex $1
